Exchange and Microviscosity of Dynamic Nanocompartments

RMs (reverse micelles) provide a controlled system for studying the unique structural and dynamic behaviors of confined water, thus gaining a general insight into the behavior or water under confinement and at interfaces. This study employs ESR (Electron Spin Resonance) to study the dynamics inside RMs and capitalizes on the fact that different preparations of RMs can precisely manipulate both the size of water pools as well as whether or not different pools can come into contact. A small spin label moiety, less than a half nanometer in size tumbles in solution, offering insight into the rotational diffusion from room temperature down to deeply super-cooled temperatures. Two different spin probes can separately probe the dynamics of the interfacial layer vs. those at the core of the reverse micelle. The results provide critical insights into how thermodynamic transitions affect the stability and behavior of water in confined spaces, enhancing the understanding of nucleation and ice crystal growth, as well as the broader understanding of confined water's role in various chemical and biological systems. The ability to more precisely understand and control reaction dynamics and thermodynamics inside confined aqueous systems across a broad range of temperatures will prove useful to fields ranging from biophysics to the development of new nano-materials.

==> acronyms.tex <==
\RequirePackage[acronyms]{glossaries}
%https://tex.stackexchange.com/questions/435617/glossaries-expand-acronyms-for-first-time-use-within-each-cha
\newacronym{oec}{OEC}{oxygen-evolving complex}
\newacronym{psii}{PSII}{Photosystem II}
\newacronym{lna}{LNA}{Low Noise Amplifier}
\newacronym{odnp}{ODNP}{Overhauser Dynamic Nuclear Polarization}
\newacronym{nmr}{NMR}{Nuclear Magnetic Resonance}
\newacronym{esr}{ESR}{Electron Spin Resonance}
\newacronym{qesr}{QESR}{Quantitative Electron Spin Resonance}
\newacronym{deer}{DEER}{Double Electron-Electron Resonance}
\newacronym{pds}{PDS}{Pulse Dipolar Spectroscopy}
\newacronym{psd}{PSD}{Power Spectral Density}
\newacronym{eseem}{ESEEM}{Electron Spin Echo Envelope Modulation}
\newacronym{sdsl}{SDSL}{Site-Directed Spin-Labeling}
\newacronym{pre}{PRE}{Paramagnetic Relaxation Enhancement}
\newacronym{awg}{AWG}{Arbitrary Waveform Generation}
\newacronym{br}{BR}{bacteriorhodopsin}
\newacronym{pr}{PR}{proteorhodopsin}
\newacronym{md}{MD}{molecular dynamics}
\newacronym{mtsl}{MTSL}{\textit{S}-(1-oxyl-2,2,5,5-tetramethyl-2,5-dihydro-1H-pyrrol-3-yl)methyl methanesulfonothioate)}
\newacronym{ednmr}{EDNMR}{electrically detected \gls{nmr}}
\newacronym{mmm}{MMM}{the open-source Matlab tool known as Multiscale Modeling of Macromolecules}
%\newacronym{pi}{PI}{principal investigator}
\newacronym{ddm}{DDM}{n-Dodecyl-β-D-Maltopyranoside}
\newacronym{dppc}{DPPC}{dipalmitoylphosphatidylcholine}
\hyphenation{dipalmitoyl-phosphatidyl-choline}
\newacronym{dopa}{DOPA}{dioleoylphosphatidic acid}
\hyphenation{di-oleoyl-phosphatidic acid}
\newacronym{sdr}{SDR}{software-defined radio}
\newacronym{avhe}{AVHE}{Academic Virtual Hosting Environment}
\newacronym{pcet}{PCET}{proton-coupled electron transfer}
\newacronym{rnr}{RNR}{Ribonuclease reductase}
\newacronym{iq}{IQ}{quadrature}
\newacronym{sasa}{SASA}{solvent-accessible surface area}
\newacronym{mr}{MR}{Magnetic Resonance}
\newacronym{dcct}{DCCT}{domain colored coherence transfer}
\newacronym{ct}{CT}{coherence transfer}
\newacronym{lp}{LP}{Linear Prediction}
\newacronym{mw}{μw}{microwave} 
\newacronym{fid}{FID}{free induction decay}
\newacronym{rm}{RM}{reverse micelle}
\newacronym{rms}{RMs}{reverse micelles}
\newacronym{snr}{SNR}{signal to noise ratio}
\newacronym{fwhm}{FWHM}{full-width-half-maximum}
\newacronym{l2g}{L2G}{Lorentzian-to-Gaussian}
\newacronym{aot}{AOT}{Aerosol-OT}
\newacronym{svd}{SVD}{Singular Value Decomposition}
\newacronym{pca}{PCA}{Principal Component Analysis}
\newacronym{sde}{SDE}{Stokes-Debye-Einstein}
\newacronym{dls}{DLS}{Dynamic Light Scattering}
\newacronym{ctet}{\ensuremath{\text{CCl}_{4}}}{carbon tetrachloride}
\newacronym{peg}{PEG}{polyethylene glycol}
\newacronym{bsa}{BSA}{bovine serum albumin}
\newacronym{ilt}{ILT}{Inverse Laplace Transform}
\newacronym{dss}{DSS}{sodium trimethylsilylpropanesulfonate}
\newacronym{ctab}{CTAB}{cetrimonium bromide}
\newacronym{sw}{SW}{spectral width}
\newacronym{fir}{FIR}{finite impulse response}
\newacronym{emi}{EMI}{electromagnetic interference}
%g!/^%*\\.*\(paragraph\|section\)/s/[{:a-zA-Z]\@<!\([A-Z]\{2,}\)[}:a-zA-Z0-9]\@!/\\gls{\L\1}/g
% and non-expanded acronyms:
%s/\\gls{\(pi\|foa\)}/\U\1/g

